Comparison of classical and Bayesian imaging in radio interferometry

CLEAN, the commonly employed imaging algorithm in radio interferometry, suffers from a number of shortcomings: in its basic version it does not have the concept of diffuse flux, and the common practice of convolving the CLEAN components with the CLEAN beam erases the potential for super-resolution; it does not output uncertainty information; it produces images with unphysical negative flux regions; and its results are highly dependent on the so-called weighting scheme as well as on any human choice of CLEAN masks to guiding the imaging. Here, we present the Bayesian imaging algorithm resolve which solves the above problems and naturally leads to super-resolution. We take a VLA observation of Cygnus~A at four different frequencies and image it with single-scale CLEAN, multi-scale CLEAN and resolve. Alongside the sky brightness distribution resolve estimates a baseline-dependent correction function for the noise budget, the Bayesian equivalent of weighting schemes. We report noise correction factors between 0.4 and 429. The enhancements achieved by resolve come at the cost of higher computational effort.

==> chisqmswgt.tex <==
\begin{tabular}{lrrr}
\hline\hline Data set & resolve & ssclean & msclean\\\hline
2052-2MHz  & 4499, 202 & 1873, 1891 & 2960, 2977\\ 4811-8MHz  & 771, 130 & 160, 151 & 291, 269\\ 8427-8MHz  & 70, 29 & 76, 25 & 113, 52\\ 13360-8MHz  & 44, 21 & 78, 31 & 136, 67\\ \hline \end{tabular}

